Near-optimal Offline and Streaming Algorithms for Learning Non-Linear Dynamical Systems

We consider the setting of vector valued non-linear dynamical systems $X_{t+1} = \phi(A^* X_t) + \eta_t$, where $\eta_t$ is unbiased noise and $\phi : \mathbb{R} \to \mathbb{R}$ is a known link function that satisfies certain {\em expansivity property}. The goal is to learn $A^*$ from a single trajectory $X_1,\cdots,X_T$ of {\em dependent or correlated} samples. While the problem is well-studied in the linear case, where $\phi$ is identity, with optimal error rates even for non-mixing systems, existing results in the non-linear case hold only for mixing systems. In this work, we improve existing results for learning nonlinear systems in a number of ways: a) we provide the first offline algorithm that can learn non-linear dynamical systems without the mixing assumption, b) we significantly improve upon the sample complexity of existing results for mixing systems, c) in the much harder one-pass, streaming setting we study a SGD with Reverse Experience Replay ($\mathsf{SGD-RER}$) method, and demonstrate that for mixing systems, it achieves the same sample complexity as our offline algorithm, d) we justify the expansivity assumption by showing that for the popular ReLU link function -- a non-expansive but easy to learn link function with i.i.d. samples -- any method would require exponentially many samples (with respect to dimension of $X_t$) from the dynamical system. We validate our results via. simulations and demonstrate that a naive application of SGD can be highly sub-optimal. Indeed, our work demonstrates that for correlated data, specialized methods designed for the dependency structure in data can significantly outperform standard SGD based methods.

==> sgd_dd.tex <==
%

\section{Analysis of SGD-DD}
\label{sec:sgd_dd_analysis}

We want to prove Theorem~\ref{thm:non_expansive_ub} by analyzing SGD-DD (Algorithm~\ref{alg:sgd-dd}). Following the approach of~\cite{nagaraj2020least}, we will show that when we take the gap $u$ to be large enough, then the data looks approximately independent. Consider the coupled process defined in Definition~\ref{def:coupled_proc} with $B = 1$ and $ u \in \mathbb{N}$ to be set later. The strategy behind the proof is as follows: 
\begin{enumerate}
\item We will first show that when $u$ is large enough, running the process with $(X_{\tau})$ is approximately same as running the process with $(\tilde{X}_{\tau})$. 
\item Since $(\tilde{X}_{\tau u})$ are independent from the stationary distribution of the process, we will use standard Lyapunov analysis for convex SGD to obtain the bounds.
\end{enumerate}
\dn{fix row wise notation for modified newton step.}
We again consider the algorithm row by row  and use the notation established in Definition~\ref{def:row_decomp}. Using this, the SGD-DD update (Algorithm~\ref{alg:sgd-dd}) becomes:

$$a_{t+1}-a^{*}= \Pi_{\mathcal{W}}\left[a_t  - 2\gamma_t\left( \sigma(\langle a_{t},X_{tu}\rangle) - \sigma(\langle a^{*},X_{tu}\rangle)\right)X_{tu} + 2\gamma_t\epsilon_{tu}X_{tu}\right] - a^{*}\,.$$
Using convexity of $\mathcal{W}$, we write:

\begin{align}
\|a_{t+1}-a^{*}\|^2 &\leq \|a_t - a^{*}\|^2 - 4\gamma_t\left( \sigma(\langle a^{t},X_{tu}\rangle) - \sigma(\langle a^{*},X_{tu}\rangle)\right)  \langle X_{tu},a_t - a^{*}\rangle  \nonumber\\&\quad + 4\gamma_t^2 \|X_{tu}\|^2|\sigma(\langle a_{t},X_{tu}\rangle) - \sigma(\langle a^{*},X_{tu}\rangle)|^2  + 4\gamma_t^2|\epsilon_{tu}|^2\|X_{tu}\|^2 \nonumber\\&\quad + 4\gamma_t^2 \epsilon_t \|X_{tu}\|^2|\sigma(\langle a_{t+1},X_{tu}\rangle) - \sigma(\langle a^{*},X_{tu}\rangle)|^2 + 2\gamma_t\epsilon_t \langle X_{tu},a_{t} - a^{*} \rangle \label{eq:sgd_recursion_1}
\end{align}
\dn{$D = \diam(\mathcal{W})$ - define this}
We note that $4\gamma_t^2 \epsilon_t \|X_{tu}\|^2|\sigma(\langle a_{t},X_{tu}\rangle) - \sigma(\langle a^{*},X_{tu}\rangle)|^2 + 2\gamma_t\epsilon_t \langle X_{tu},a_{t} - a^{*} \rangle$ has zero expectation. We also note that $4\gamma_t^2\mathbb{E}|\epsilon_{tu}|^2\|X_{tu}\|^2 = 4\gamma_t^2\sigma^2\mathbb{E}\|X_{tu}\|^2$. 



By $\hat{\loss}_t$ we denote $\mathbb{E}\left( \sigma(\langle a^{t+1},X_{tu}\rangle) - \sigma(\langle a^{*},X_{tu}\rangle)\right)  \langle X_{tu},a_t - a^{*}\rangle $.  Since $\sigma$ is non-decreasing and $1$ Lipschitz, we conclude that $\left( \sigma(\langle a^{t},X_{tu}\rangle) - \sigma(\langle a^{*},X_{tu}\rangle)\right)\langle X_{tu},a_t - a^{*}\rangle \geq  |\sigma(\langle a^{t},X_{tu}\rangle) - \sigma(\langle a^{*},X_{tu}\rangle)|^2$. Define the event $\mathcal{D}_{tu}(R) := \{\|X_{tu}\|^2 \leq R\}$ for some $R >0$. We have:  

\begin{align}
\mathbb{E}\|X_{tu}\|^2|\sigma(\langle a_{t},X_{tu}\rangle) - \sigma(\langle a^{*},X_{tu}\rangle)|^2  &\leq \mathbb{E}R^2\mathbbm{1}(\mathcal{D}_{tu}(R))|\sigma(\langle a_{t},X_{tu}\rangle) - \sigma(\langle a^{*},X_{tu}\rangle)|^2  \nonumber\\&\quad +  \mathbb{E}\|X_{tu}\|^4\|a_t - a^{*}\|^2 \mathbbm{1}(\mathcal{D}_{tu}^c(R)) \nonumber \\
&\leq R \mathbb{E}|\sigma(\langle a_{t},X_{tu}\rangle) - \sigma(\langle a^{*},X_{tu}\rangle)|^2 \nonumber\\&\quad+ D^2\sqrt{\mathbb{P}(\mathcal{D}_{tu}^c(R))}\sqrt{\mathbb{E}\|X_{tu}\|^{8}} \nonumber \\
&\leq  R \mathbb{E}\left( \sigma(\langle a^{t},X_{tu}\rangle) - \sigma(\langle a^{*},X_{tu}\rangle)\right)\langle X_{tu},a_t - a^{*}\rangle \nonumber\\&\quad+ D^2\sqrt{\mathbb{P}(\mathcal{D}_{tu}^c(R))}\sqrt{\mathbb{E}\|X_{tu}\|^{8}} \nonumber \\
&= R \hat{\loss}_t + D^2\sqrt{\mathbb{P}(\mathcal{D}_{tu}^c(R))}\sqrt{\mathbb{E}\|X_{tu}\|^{8}} \label{eq:smoothness_bound}
\end{align}
Taking expectation in Equation~\eqref{eq:sgd_recursion_1}, and using the bound in Equation~\eqref{eq:smoothness_bound}, we obtain that:

\begin{align}
\mathbb{E}\|a_{t+1}-a^{*}\|^2  \leq \mathbb{E}\|a_t - a^{*}\|^2 - \left(2\gamma_t - 4R\gamma_t^2 \right)\hat{\loss}_t + 4\gamma_t^2D^2\sqrt{\mathbb{P}(\mathcal{D}_{tu}^c(R))}\sqrt{\mathbb{E}\|X_{tu}\|^{8}} + 4\gamma_t^2 \sigma^2 \mathbb{E}\|X_{tu}\|^2\label{eq:lyapunov_recursion}
\end{align}
\dn{change this to frobenius norm projection instead}
Now, we sum the Equation~\eqref{eq:lyapunov_recursion} from $t=0$ to $t= T/u$.
\begin{equation}\label{eq:final_recursion}
\sum_{t=0}^{T/u} \left(2\gamma_t -4R\gamma_t^2\right)   \hat{\loss}_t  \leq D^2 + \left(D^2\sqrt{\mathbb{P}(\mathcal{D}_{tu}^c(R))}\sqrt{\mathbb{E}\|X_{tu}\|^{8}} + \sigma^2 \mathbb{E}\|X_{tu}\|^2 \right)\sum_{t=0}^{T/u + 1}4\gamma_t^2
\end{equation}

We will use the arguments succeeding Equation~\eqref{eq:fourth_moment_bound_1} to show that when we pick $R = R^{*} = \bar{C}\sigma^2 \frac{d}{1-\rho}\log \left(\tfrac{d}{1-\rho}\right)$, where $\bar{C}$ is a constant depending only on $C_{\eta}$, we have:
$D^2\sqrt{\mathbb{P}(\mathcal{D}_{tu}^c(R))}\sqrt{\mathbb{E}\|X_{tu}\|^{8}} \leq D^2 \bar{C}_1\frac{\sigma^4d}{1-\rho}\,.$
From Theorem~\ref{thm:process_concentration}, we have that $\mathbb{E}\|X_{tu}\|^4 \leq \bar{C}_2 \frac{\sigma^2 d}{1-\rho}$. Using these in Equation~\eqref{eq:final_recursion} we show that:


\begin{equation}\label{eq:final_recursion_1}
\sum_{t=0}^{T/u} \left(2\gamma_t -4R^{*}\gamma_t^2\right)   \hat{\loss}_t  \leq D^2 + (D^2+1)\frac{\bar{C}\sigma^4 d}{1-\rho}\sum_{t=0}^{T/u + 1}4\gamma_t^2
\end{equation}


We will show that since $\tilde{X}_{tu}\approx X_{tu}$ and $a_t$ is independent of $\tilde{X}_{tu}$, we have $\hat{\loss}_t$ to be close to the generalization error. Now, by assumption, we have constant step size $\gamma_t = \gamma$ and $4R^{*}\gamma < 1$. From Equation~\eqref{eq:final_recursion_1} we conclude that:


==> uniformly_bounded_ar.tex <==
%
\section{Uniformly Bounded GLMs Can Be Recovered With SGD}
 Suppose $\nu \in \mathbb{R}^d$ be fixed and known such that $\|\nu\|_{\infty} \leq \numax$. Consider $\A \in \mathbb{R}^{d\times d}$ to be the unknown matrix to be estimated. Let $a_i^{*} \in \mathbb{R}^d$ be the vector corresponding to the i-th row of $\A$ (but written in the column form). We let $X_0 \in \Omega \subseteq \mathbb{R}^d$ be arbitrary. We suppose that $M := \sup_{x\in \Omega}\|x\|_{\infty} < \infty$. Suppose $\sigma :\mathbb{R} \to \mathbb{R}$ is a continuously differentiable, increasing function. We now consider the stochastic process $X_0,X_1,\dots, X_T \in \Omega$ a.s. such that:
 
 $$X_{t+1} = \sigma(\nu + \A X_t) + \eta_t \,.$$
Here the scalar function $\sigma$ is assumed to act component wise in the standard basis on vectors, $\eta_t$ is a vector such that $\mathbb{E}\left[ \eta_t|X_t,\dots,X_0\right] = 0$. Here, we assume that $\eta_t$ is such that the trajectory is in the bounded set $\Omega$ almost surely and that $\|\eta_t\|_{\infty} \leq M$. Let us fix a parameter $\gamma $ such that $\|\A\|_{\infty} < \gamma$. This is equivalent to the condition. $\sup_i \|a_i^{*}\|_1 < \gamma$. %We also suppose that we know the sparsity pattern of $A^{*}$. That is for each row, $a_i^{*}$ of $A^{*}$, we know the set $S_i \subseteq [d]$ such that $A^{*}_{ij} = 0$ for every $j \in S_i^{c}$.
We let $\mathcal{W}_{\gamma} \subseteq \mathbb{R}^d$ be the closed $\ell^1$ ball of radius $\gamma$.  By $\Pi_{\gamma}$, we denote the projection operator to the set $\mathcal{W}_{\gamma}$. We consider projected SGD for recovering the parameter $\A$ row by row as follows. For simplicity we run the $t$-th step with data $(X_{2t},X_{2t+1})$.


\begin{enumerate}
    \item Fix a horizon $T$ and a step size sequence $\alpha_t >0$. 
    \item Let $a_i(0) \in \mathbb{R}^{d}$.  
    \item Update:
    $$a_i(t+1) = \Pi_{\gamma}\left(a_i(t) - \alpha_t \left[\sigma(\nu_i + \langle a_i(t),X_{2t}\rangle) - X_{2t+1,i}\right] X_{2t}\right)$$
\end{enumerate}



\begin{assumption}[Restricted Lipschitzness]
We assume that $\sup_{|x| \leq \numax+\gamma} \sigma^{\prime}(x) \leq  \beta$.
\end{assumption}

\begin{assumption}[Restricted Expansivity]
We assume that $\inf_{|x| \leq \numax+\gamma} \sigma^{\prime}(x) \geq \zeta$.
\end{assumption}
Consider $\mathcal{F}_t = \sigma(X_0,\dots,X_t)$, the natural filtration associated with the process $X_0,X_1,\dots,X_T$.
\begin{assumption}[Iterative Well Conditioning]
$\mathbb{E} X_{t+1}X_{t+1}^{\intercal} \succeq c_0 I$ for some $c_0 > 0$
\end{assumption}
We can now write down the update equations as: $$a_i(t+1)= \Pi_{\gamma}\left(a_i(t) - \alpha_t\left[ \sigma(\nu_i + \langle a_i(t),X_{2t}\rangle) - \sigma(\nu_i +\langle a_i^{*},X_{2t}\rangle) \right] X_{2t} + \alpha_t \eta_{2t,i} X_{2t}\right)\,.$$
Therefore:
\begin{align}
 \|a_i(t+1)-a_i^{*}\|^2 &\leq   \|a_i(t)-a_i^{*}\|^2 - 2\alpha_t\langle\left[ \sigma(\nu_i + \langle a_i(t),X_{2t}\rangle) - \sigma(\nu_{i} +\langle a_i^{*},X_{2t}\rangle) \right] X_{2t},a_i(t)-a_i^{*} \rangle \nonumber \\&\quad + 2\alpha_t \langle \eta_{2t,i}  X_{2t}, a_i(t)-a_i^{*}\rangle \nonumber \\ &\quad+ 2\alpha_t^{2}\langle \eta_{2t,i}X_{2t}, \left[ \sigma(\nu_i + \langle a_i(t),X_{2t}\rangle) - \sigma(\nu_{i} +\langle a_i^{*},X_{2t}\rangle) \right]X_{2t} \rangle \nonumber \\ &\quad+  \alpha_t^{2}|\eta_{2t,i}|^2\|X_{2t}\|^2 + \alpha_t^{2}\|X_{2t}\|^2 | \sigma(\nu_i + \langle a_i(t),X_{2t}\rangle) - \sigma(\nu_{i} +\langle a_i^{*},X_{2t}\rangle) |^2 
\end{align}
Now, the terms:
$ 2\alpha_t \langle \eta_{2t,i} X_{2t}, a_i(t) -a_i^{*}\rangle + 2\alpha_t^{2}\langle \eta_{2t,i}X_{2t}, \left[ \sigma(\nu_i + \langle a_i(t),X_{2t}\rangle) - \sigma(\nu_{i} +\langle a_i^{*},X_{2t}\rangle) \right]X_{2t} \rangle$ have $0$ expectation. Therefore, we conclude:

\begin{align}
   \mathbb{E}\|a_i(t+1)-a_i^{*}\|^2 &\leq  \mathbb{E} \|a_i(t)-a_i^{*}\|^2 - 2\alpha_t\mathbb{E} \langle\left[ \sigma(\nu_i + \langle a_i(t),X_{2t}\rangle) - \sigma(\nu_{i} +\langle a_i^{*},X_{2t}\rangle) \right]X_{2t},a_i(t)-a_i^{*} \rangle  \nonumber \\ &\quad+  \alpha_t^{2}\mathbb{E}|\eta_{2t,i}|^2\|X_{2t}\|^2 + \mathbb{E}\alpha_t^{2}\|X_{2t}\|^2 |\sigma(\nu_i + \langle a_i(t),X_{2t}\rangle) - \sigma(\nu_{i} +\langle a_i^{*},X_{2t}\rangle)|^2 \nonumber \\
   &\leq \mathbb{E} \|a_i(t)-a_i^{*}\|^2 - 2\alpha_t\mathbb{E} \langle\left[ \sigma(\nu_i + \langle a_i(t),X_{2t}\rangle) - \sigma(\nu_{i} +\langle a_i^{*},X_{2t}\rangle) \right]X_{2t},a_i(t)-a_i^{*} \rangle  \nonumber \\ &\quad+  \alpha_t^{2}(L^2M^2 + 4M^4)d
   \end{align}
Now we will use iterative well conditioning to bound the quantity: $$\mathbb{E} \langle\left[ \sigma(\nu_i + \langle a_i(t),X_{2t}\rangle) - \sigma(\nu_{i} +\langle a_i^{*},X_{2t}\rangle) \right] X_{2t},a_i(t)-a_i^{*} \rangle$$

\begin{lemma}\label{lem:iterative_contraction}
$$\mathbb{E}\left[\left[ \sigma(\nu_i + \langle a_i(t),X_{2t}\rangle) - \sigma(\nu_{i} +\langle a_i^{*},X_{2t}\rangle) \right]X_{2t},a_i(t)-a_i^{*} \rangle|\mathcal{F}_{2t-1}\right] \geq \zeta c_0  \|a_i(t) - a_i^{*}\|^2$$
\end{lemma}

\begin{proof}
First, we conclude by the mean value theorem that:

\begin{align}
    &\langle\left[ \sigma(\nu_i + \langle a_i(t),X_{2t}\rangle) - \sigma(\nu_{i} +\langle a_i^{*},X_{2t}\rangle) \right]X_{2t},a_i(t)-a_i^{*} \rangle \nonumber \\ &= \sigma^{\prime}(l_t) (a_i(t) - a_i^{*})^{\intercal} X_{2t} X_{2t}^{\intercal}(a_i(t) - a_i^{*}) \nonumber \\
    &\geq \zeta (a_i(t) - a_i^{*})^{\intercal} X_{2t} X_{2t}^{\intercal}(a_i(t) - a_i^{*}) \nonumber \\
\end{align}

It is easy to show that $a_i(t)$ is $\mathcal{F}_{2t-1}$ measurable. Therefore, taking conditional expectation, we have:

\begin{align}
 \mathbb{E}\left[(a_i(t) - a_i^{*})^{\intercal} X_{2t} X_{2t}^{\intercal}(a_i(t) - a_i^{*})|\mathcal{F}_{2t-1}\right] 
&= (a_i(t) - a_i^{*})^{\intercal}\mathbb{E}\left[ X_{2t} X_{2t}^{\intercal}|\mathcal{F}_{2t-1}\right](a_i(t) - a_i^{*}) \nonumber \\
&\geq c_0 \|a_i(t)-a_i^{*}\|^2
\end{align}
From the two equations above, we conclude the statement of the lemma.
\end{proof}


Therefore, applying Lemma~\ref{lem:iterative_contraction}, we conclude:

\begin{align}
   \mathbb{E}\|a_i(t+1)-a_i^{*}\|^2 
   &\leq \mathbb{E} \|a_i(t)-a_i^{*}\|^2(1 - 2\alpha_t c_0\zeta)+  \alpha_t^{2}(L^2M^2 + 4M^4)d
\end{align}
   
Picking the step size to be $\alpha_t = \frac{1}{2c_0 \zeta(t+1)}$ shows that for $t \geq 0$ we have by an inductive proof similar to Lemma 1 in~\cite{rakhlin2012making}.
\begin{theorem}\label{thm:bounded_ar_sgd}
$$\mathbb{E}\|a_i(t+1)-a_i^{*}\|^2 \leq \frac{(L^2M^2 + 4M^4)d}{4c_0^{2}\zeta^2 t}$$ 
\end{theorem}

\subsection{Bernoulli Autoregressive Model}



We now consider the case of Bernoulli auto regressive model. Consider the following stochastic process over $\{0,1\}^{d}$. Let $X_{0}\in \{0,1\}^d$ be arbitrary. We then draw $X_{t+1}(i) \sim \ber(\sigma(\nu(i) + \langle a_i^{*},X_t\rangle)) $ where $\sigma(x) := \frac{1}{1+e^{-x}}$. We can then write $X_{t+1} = \sigma(\nu + \A X_t) + \eta_t$ where the scalar function $\sigma$ is understood to act co-ordinate wise on a vector. Here, $\eta_t$ is a $0$ zero mean vector whose distribution depends only on the value of $X_t$ and we have $\mathbb{E}\left[\eta_t|X_t\right] = 0$. In this case, $L=M=1$. We need to show the assumptions preceding the theorem holds in this case too. Clearly, $\sigma$ is a strictly increasing function, 1 Lipschitz function. $\sigma^{\prime}(x) = \sigma(x)(1-\sigma(x)) $, Therefore, $\inf_{|x| \leq \numax + \gamma}\sigma^{\prime}(x) \geq \frac{1}{4}\exp(-\numax-\gamma)$. We can take $\zeta = \frac{1}{4}\exp(-\numax-\gamma)$. Now, we will show iterative well conditioning property (Similar to Theorem 6 in \cite{hall2018learning}). Clearly, $\mathbb{E}\left[X_{t+1}X_{t+1}^{\intercal}|X_t\right]\succeq \mathbb{E}\left[\eta_t\eta_t^{\intercal}|X_t\right]$. Now, consider for $i\neq j$ and $i,j \in [d]$: $\mathbb{E}\left[\eta_{t,i}\eta_{t,j}|X_t\right] = 0$ and $\mathbb{E}\left[\eta_{t,i}^2|X_t\right] = \sigma(\nu_i + \langle a^{*}_i,X_t\rangle)(1- \sigma(\nu_i + \langle a^{*}_i,X_t\rangle)) \geq \frac{1}{4}\exp(-\numax-\gamma)$.
Therefore, we can take $c_0 = \frac{1}{4}\exp(-\numax-\gamma)$. Plugging this in Theorem~\ref{thm:bounded_ar_sgd}, we conclude:
\begin{proposition}
For the Bernoulli Auto Regressive model, we have for some universal constant $C$: 
$$\mathbb{E}\|a_i(T/2)-a_i^{*}\|^2 \leq \frac{C\exp(4\numax+4\gamma)d}{ T}$$ 
\end{proposition}
